A Churn for the Better: Localizing Censorship using Network-level Path Churn and Network Tomography

Recent years have seen the Internet become a key vehicle for citizens around the globe to express political opinions and organize protests. This fact has not gone unnoticed, with countries around the world repurposing network management tools (e.g., URL filtering products) and protocols (e.g., BGP, DNS) for censorship. However, repurposing these products can have unintended international impact, which we refer to as "censorship leakage". While there have been anecdotal reports of censorship leakage, there has yet to be a systematic study of censorship leakage at a global scale. In this paper, we combine a global censorship measurement platform (ICLab) with a general-purpose technique -- boolean network tomography -- to identify which AS on a network path is performing censorship. At a high-level, our approach exploits BGP churn to narrow down the set of potential censoring ASes by over 95%. We exactly identify 65 censoring ASes and find that the anomalies introduced by 24 of the 65 censoring ASes have an impact on users located in regions outside the jurisdiction of the censoring AS, resulting in the leaking of regional censorship policies.

==> Makefile <==
# Makefile for LaTeX files

# Original Makefile from http://www.math.psu.edu/elkin/math/497a/Makefile

# Please check http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# for new versions.

# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

# $Id: Makefile,v 1.18 2006-06-19 10:58:11 mairas Exp $

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex
XDVI	= xdvi -gamma 4
DVIPS	= dvips
DVIPDF  = dvipdft
L2H	= latex2html
GH	= gv

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false

# These are OK

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG	= $(SRC:%.tex=%.dvi)
PSF	= $(SRC:%.tex=%.ps)
PDF	= $(SRC:%.tex=%.pdf)

# These are not

#BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))
#DEP     := $(shell perl -ne '($$_)=/^[^%]*\\include\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $(SRC))
#EPSPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $(SRC) $(DEP))


define run-latex
	$(COPY);$(LATEX) $<
	egrep $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) >/dev/null; true
	egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	egrep $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) >/dev/null; true
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	$(RM) $(<:%.tex=%.toc.bak)
	# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

define run-pdflatex
	LATEX=pdflatex
	@$(run-latex)
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define geteps
	epses=`perl -ne '@foo=/^[^%]*\\\(includegraphics|psfig)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$$foo[2] "; } else { print "$$foo[2].eps "; }}' $< $$deps`
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef

all 	: $(TRG)

.PHONY	: all show clean ps pdf showps veryclean

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.dvi=%.aux) $(TRG:%.dvi=%.bbl) $(TRG:%.dvi=%.blg) $(TRG:%.dvi=%.log) $(TRG:%.dvi=%.out) $(TRG:%.dvi=%.idx) $(TRG:%.dvi=%.ilg) $(TRG:%.dvi=%.ind) $(TRG:%.dvi=%.toc) $(TRG:%.dvi=%.d)

veryclean	: clean
	  -rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.ps  *~

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	$(get_dependencies) ; echo $$deps ; \
	$(getbibs) ; echo $$bibs ; \
	$(manconf) ; echo  $$mandeps  ;\
	echo "$*.dvi $@ : $< $$deps $$bibs $$epses $$mandeps" > $@ 

include $(SRC:.tex=.d)

# $(DEP) $(EPSPICS) $(BIBFILE)
$(TRG)	: %.dvi : %.tex
	  @$(run-latex)

$(PSF)	: %.ps : %.dvi
	  @$(DVIPS) $< -o $@

#$(PDF)  : %.pdf : %.dvi
#	  @$(DVIPDF) -o $@ $<
# To use pdflatex, comment the two lines above and uncomment the lines below
$(PDF) : %.pdf : %.tex
	@$(run-pdflatex)


show	: $(TRG)
	  @for i in $(TRG) ; do $(XDVI) $$i & done

showps	: $(PSF)
	  @for i in $(PSF) ; do $(GH) $$i & done

ps	: $(PSF) 

pdf	: $(PDF) 

# TODO: This probably needs fixing
html	: @$(DEP) $(EPSPICS)
	  @$(L2H) $(SRC)



######################################################################
# Define rules for EPS source files.

# These rules probably just cause unnecessary confusion, so commenting
# them away for the time being. -- mairas 2005-01-12

#%.eps: %.sxd
#	$(OUTDATED)
#%.eps: %.sda
#	$(OUTDATED)
#%.eps: %.png
#	$(OUTDATED)
#%.eps: %.sxc
#	$(OUTDATED)
#%.eps: %.xcf
#	$(OUTDATED)
#%.eps: %.zargo
#	$(OUTDATED)
#%.eps: %.m
#	@egrep -q $(MPRINT) $< && ($(OUTDATED))


==> acknowledgements.tex <==
\section*{Acknowledgements}



==> censorship.tex <==
\section{Identifying Censors and Censorship Leakage}\label{sec:censorship}




==> map.tex <==
\section{Identifying Censors}\label{sec:isolating}
We now describe how we identify censoring ASes and censorship leakage using
measurements from the ICLab platform. At a high-level, our approach works as
follows:

\begin{itemize}
\item First, we use the traceroutes gathered by the ICLab platform to construct
boolean clauses such that the literals in the clauses represent ASes observed in
the traceroute. We then use the censorship measurements associated with the
corresponding traceroutes to assign truth values to the clauses. Finally, the
clauses are converted to Conjunctive Normal Form (CNF) and used as input to an
off-the-shelf SAT solver. The process is repeated for each type of censorship
measurement (\ie DNS injection, HTTP tampering, and blockpage detection) and
various time slices (\ie for all measurements performed during the same day,
week, and month). 
\item Next, we analyze the solutions returned by the SAT solver for each CNF. In
cases where there are multiple solutions -- \ie multiple truth assignments for a
given CNF formulation -- we return all literals (ASes) having \emph{True}
assignments as potential censors. In cases where there is a single solution, we
return all literals (ASes) having \emph{True} assignments as censors.
\item Finally, we characterize censorship leakage by identifying ASes that
exhibit similar forms of censorship only when they are present downstream from
the censoring ASes.
\end{itemize}

\subsection{Mapping ICLab data to the SAT problem}
Each record in the ICLab dataset contains: (1) the vantage point AS, (2) the URL
being tested, (3) the anomaly being tested (and whether it was detected or not),
(4) three traceroutes between the vantage point and the URL at the time of
testing, and (5) the time at which the test was performed. We use each of these
records to create boolean clauses as follows: 

\myparab{Clause formulation.} First, we use historical IP-to-AS
mapping from CAIDA \cite{ip-as-mapping} to convert the IP-level traceroutes to
AS-level paths. Next, we eliminate cases with inconclusive paths -- \ie cases
where one of the following situations occurred: (1) IP-to-AS mapping was not
possible for any of the IPs observed in the traceroute, (2) traceroutes were not
possible due to errors, (3) AS-inference was not possible due to non-responsive
hops and different ASes observed in the previous and subsequent responsive hop,
and (4) there was more than one AS-level path obtained after conversion of the
three traceroutes. Each of the remaining AS-level paths forms a clause in our
SAT formulation, with each observed AS acting as a literal. The truth value
attached to the clause is \emph{True} if the measurement detected its
corresponding anomaly, and \emph{False} otherwise. For example, if the
AS-level path $X \rightarrow Y \rightarrow Z$ observed DNS censorship, it is
represented by the clause $(X_{DNS} \lor Y_{DNS} \lor Z_{DNS}) = T$. 

\myparab{Time-based splitting.} Our formulation accounts for the fact that
censorship policies and techniques may change over time  (\eg Iran is known to
increase censorship during political events such as elections
\cite{Aryan-FOCI13}). Not doing so introduces the possibility of generating an
unsolvable CNF in the event of a policy change -- \eg the measurement $(X_{DNS}
\lor Y_{DNS} \lor Z_{DNS}) = T$ is observed on Day 1 and $(X_{DNS} \lor Y_{DNS}
\lor Z_{DNS}) = F$ on Day 2. We address this problem by creating CNFs at four
time granularities -- days, weeks, months, and year. We generate one CNF for
each day, week, month, and year contained in the ICLab data. Finally, each CNF
is solved using and off-the-shelf SAT solver.

%\myparab{Sample.} In this section, we map our problem to Boolean satisfiability
%problem. When a set of paths and their analyzed anomaly states (normal or
%anomaly) are given, we create a Boolean formula to run our solver. We provide a
%simple example in Figure \ref{fig:sample}
%
%\begin{figure}
%	\includegraphics[clip=true,width=.400\textwidth]
%	{figures/sample.png}
%	\caption{A simple example.}
%	\label{fig:sample}
%\end{figure}
%
%The example has two paths $P_j$ ($j=1,2$) and nodes $v_i$ ($i=1,\dots,5$). Each
%path can have a state of \{0, 1\}, or we can say \{normal, anomaly\}, and each
%node can have one state of \{0, 1\} or \{false, true\}. In the example, $P_1 =
%v_1,v_2,v_4,v_5$ is a normal path with a state \{0\}. On the other hand, $P_2 =
%v_1,v_2,v_3,v_5$ is an anomaly path with a state \{1\}. Given this information,
%we create clauses from all paths and formulate a Boolean formula followed by
%conjunctive normal form (CNF). Then, we run this formula to our solver and get a
%result.
%
%Lets see the process of creating clauses and a formula in details. We generate a
%clause based on two different states of paths. For a true path, $P_2$, we
%generate a clause as $(v_1 \lor v_2 \lor v_3 \lor v_5)$. For a false path,
%$P_1$, we generate clauses as $(\neg v_1), (\neg v_2), (\neg v_4), (\neg v_5)$.
%Then, we generate a final Boolean formula as a conjunction of all clauses such
%that: 
%
%\begin{equation}  
% (v_1 \lor v_2 \lor v_3 \lor v_5) \land
% (\neg v_1) \land (\neg v_2) \land (\neg v_4) \land (\neg v_5)
%\end{equation}
% 
%To find a satisfying assignment for the formula, at least one variable in the
%$P_2$ clause should be a true value. It means that at least one node in $P_2$ is
%the cause of path change and is responsible for the analyzed anomaly. At the
%same time, all variables in $P_1$ clauses should be false value to make the
%formula satisfiable, which means that all nodes in $P_1$ are not the cause of
%path changes. Finally, our Sat solver returns \{$v_3$\} as a candidate node
%responsible for anomaly with the formula (1).   
%
% 
%\myparab{Generilization.} We generalize our Boolean formula to use. Let nodes be
%$v_1, v_2, v_3, \dots, v_n \in \{0, 1\}$ (or \{true, false\}) and paths $P_1,
%P_2, \dots, P_N$. Each path has analyzed path state $s_1, s_2, \dots, s_N \in
%\{0,1\}$ (or \{normal, anomaly\}). Given this information, We generate clauses
%$c_i$ for a path $Pi = v_1,v_2,...,vk$ with its state $s_i$, as follows:
% 
%\begin{equation}
%	c_i=
%	\begin{cases}
%	(v_1 \lor v_2 \lor \dots \lor v_k), & \text{if } s_i \text{ is 1, and} \\
%	(\neg v_1) \lor (\neg v_2) \lor \dots \lor (\neg v_k) & \text{if } s_i \text{ is 0}  
%	\end{cases}
%\end{equation}
%After we get all clauses, we formulate a Boolean formula $B$ as a conjunction of
%clauses, as follows:
%\begin{equation}
%	B=\land_{i=1}^{n}c_{i}
%\end{equation}
%Then, our Sat solver finds the satisfying assignment that minimizes the number
%of true variables.
% 
%
%\myparab{Discussion.}
% Note that we are limited by the noise present in the input dataset. This
%restricts our SAT system solvability. 
%
%\young{Todo: Specifically demonstrate examples where multiple or no solutions
%may exist and what this implies.}
%
%\subsection{Validation experiment}
%
%\myparab{Validation experiment: Measuring network churn over time.}
%Our approach is contingent on there being enough network-level path-churn. We
%need to show that this is indeed the case. Describe the experiment and results
%that show the number of paths observed between each recorded source and
%destination over varying periods of time. Also good to break it down by AS type
%so we can identify the types of problems that can be solved by our approach.
%If its possible to characterize where in the path churn is observed, that will
%also be very useful!
%
%\section{Identifying Network-level Censors}\label{sec:censorship}
%
%\myparab{Solvability experiment.} How many of our cases where actually solvable?
%Identify few interesting cases that were not solvable and hypothesize why this
%was the case. Show how solvability increases as the size of the time slice
%reduces. Also make sure its clear that solvability does not imply a definite
%single solution -- multiple solutions may exist.
%
%\myparab{Suspected censors experiment.} Specifically analyze only the solvable
%cases. How many times were we able to exactly identify the censors (\ie cases
%with only one solution)? In the cases that exact identification was not possible
%(\ie we had multiple solutions), how much were we able to reduce the suspect set
%size by (use ratios)? 
%
%\myparab{Identified censors.} Now we'll take a look at the specific (definite)
%censors that we identified. Make a table that describes their region of
%operation, the type of censorship observed, the types of content that were
%blocked -- use McAfee URL cats, how big were these censors?
%
%\myparab{Identifying censorship leakage.} How many of the above censoring ASes
%have upstream ASes that are in different regions that are also impacted by their
%censorship policies? CDF of the number of regions. Pick out the leakiest censors
%and talk about them.
%
% \subsection{Results}\label{sec:isolating:results}
% 
% Impact: time period, # of unique paths, length of as path
% Anomalies - ttl, dns, seq, block, rst
% Time - day, week, month
% Source AS - all, fix, exclusi
% AS path length - more than 2, 3, 4
% Number of unique paths
% Number of unique ASes
% Accuracy, real-time, precision, robustness, and scalability
% Verification

